Localization of Compact Binary Sources with Second Generation Gravitational-wave Interferometer Networks

GW170817 began gravitational-wave multimessenger astronomy. However, GW170817 will not be representative of detections in the coming years -- typical gravitational-wave sources will be closer the detection horizon, have larger localization regions, and (when present) will have correspondingly weaker electromagnetic emission. In its design state, the gravitational-wave detector network in the mid-2020s will consist of up to five similar-sensitivity second-generation interferometers. The instantaneous sky-coverage by the full network is nearly isotropic, in contrast to the configuration during the first \change{three} observing runs. Along with the coverage of the sky, there are also commensurate increases in the average horizon for a given binary mass. We present a realistic set of localizations for binary neutron stars and neutron star--black hole binaries, incorporating intra-network duty cycles and selection effects on the astrophysical distributions. Based on the assumption of an $80\%$ duty cycle, and that two instruments observe a signal above the detection threshold, we anticipate a median of $28$ sq.\ deg.\ for binary neutron stars, and $50$--$120$ sq.\ deg.\ for neutron star--black hole (depending on the population assumed). These distributions have a wide spread, and the best localizations, even for networks with fewer instruments, will have localizations of $1$--$10$ sq.\ deg.\ range. The full five instrument network reduces localization regions to a few tens of degrees at worst.

==> 2_det_subnet.tex <==
& HI & HK & HL & HV & IK & IL & IV & KL & KV & LV \\
\hline
BNS uniform & \intrv{287.1}{596.5}{231.6} & \intrv{348.9}{629.2}{282.0} & \intrv{1710.0}{995.8}{1303.0} & \intrv{273.4}{569.9}{229.4} & \intrv{493.0}{762.6}{382.4} & \intrv{358.5}{570.9}{293.3} & \intrv{330.1}{718.0}{269.1} & \intrv{248.6}{578.2}{191.8} & \intrv{256.3}{555.8}{205.5} & \intrv{255.7}{594.9}{202.9} \\
BNS normal & \intrv{270.5}{607.5}{234.8} & \intrv{345.1}{586.8}{276.7} & \intrv{1796.2}{953.1}{1360.6} & \intrv{241.4}{527.0}{199.1} & \intrv{463.2}{776.8}{369.6} & \intrv{376.3}{537.2}{307.9} & \intrv{320.8}{683.2}{259.6} & \intrv{246.0}{618.4}{193.4} & \intrv{260.1}{580.4}{207.6} & \intrv{239.6}{578.9}{193.7} \\
NSBH uniform & \intrv{618.5}{24810.6}{542.4} & \intrv{630.6}{23723.0}{506.8} & \intrv{2947.6}{22332.4}{2146.2} & \intrv{538.2}{28983.7}{461.3} & \intrv{839.1}{21543.1}{703.2} & \intrv{736.4}{27590.5}{624.7} & \intrv{628.1}{23637.4}{522.5} & \intrv{470.2}{25279.7}{394.7} & \intrv{452.6}{20094.0}{383.8} & \intrv{446.8}{24899.1}{368.2} \\
NSBH astro & \intrv{397.1}{6826.8}{340.5} & \intrv{452.5}{12021.4}{365.0} & \intrv{2165.2}{6196.7}{1571.3} & \intrv{330.1}{7178.0}{272.0} & \intrv{627.4}{9225.4}{508.5} & \intrv{466.2}{4711.3}{384.5} & \intrv{423.2}{15940.9}{343.1} & \intrv{332.0}{7694.8}{279.2} & \intrv{346.0}{11054.1}{274.9} & \intrv{319.2}{14317.4}{255.3} \\


==> 2g_loc.tex <==
population & 2 & 3 & 4 & 5 & 20\% & 50\% & 80\% \\ \hline
bns uniform  &  \intrv{260}{1300}{240} & \intrv{12}{72}{11} & \intrv{3.8}{13}{3.5} & \intrv{2.3}{5.6}{2.2}  &  \intrv{160}{1100}{160} & \intrv{22}{790}{21} & \intrv{3.7}{90}{3.2} \\
bns normal  &  \intrv{250}{1300}{230} & \intrv{11}{69}{10} & \intrv{3.8}{14}{3.4} & \intrv{2.1}{5.6}{2}  &  \intrv{150}{1100}{150} & \intrv{20}{780}{19} & \intrv{3.7}{83}{3.2} \\
NSBH uniform  &  \intrv{570}{4100}{520} & \intrv{45}{720}{41} & \intrv{16}{230}{15} & \intrv{9.4}{130}{8.6}  &  \intrv{380}{3200}{370} & \intrv{95}{2200}{91} & \intrv{19}{380}{17} \\
NSBH astro  &  \intrv{390}{2700}{360} & \intrv{22}{300}{20} & \intrv{6.9}{79}{6.1} & \intrv{4}{49}{3.7}  &  \intrv{260}{1900}{250} & \intrv{47}{1400}{45} & \intrv{8.2}{190}{7.4} \\


==> 3_det_subnet.tex <==
& HIK & HIL & HIV & HKL & HKV & HLV & IKL & IKV & ILV & KLV \\
\hline
BNS uniform & \intrv{54.0}{210.6}{47.4} & \intrv{94.3}{450.7}{85.5} & \intrv{51.0}{241.8}{46.2} & \intrv{217.0}{1382.5}{195.2} & \intrv{30.9}{169.6}{27.0} & \intrv{165.1}{1119.9}{156.3} & \intrv{46.2}{142.2}{40.9} & \intrv{47.8}{350.5}{42.2} & \intrv{77.2}{377.4}{71.1} & \intrv{30.7}{325.4}{26.3} \\
BNS normal & \intrv{54.3}{199.6}{47.5} & \intrv{87.0}{453.5}{77.6} & \intrv{52.6}{232.0}{46.9} & \intrv{213.9}{1492.5}{193.2} & \intrv{25.9}{156.1}{21.9} & \intrv{176.0}{1096.4}{166.5} & \intrv{51.7}{137.6}{45.9} & \intrv{47.5}{317.8}{42.4} & \intrv{73.7}{352.7}{67.6} & \intrv{35.7}{299.9}{31.7} \\
NSBH uniform & \intrv{121.0}{15477.2}{108.0} & \intrv{218.5}{11759.2}{195.1} & \intrv{142.4}{23416.1}{128.2} & \intrv{520.9}{22504.3}{476.2} & \intrv{67.4}{20608.5}{58.9} & \intrv{575.9}{29681.6}{556.0} & \intrv{125.7}{22166.5}{113.3} & \intrv{102.7}{23305.8}{91.9} & \intrv{189.6}{25481.2}{172.4} & \intrv{81.1}{27454.5}{73.5} \\
NSBH astro & \intrv{70.6}{2170.1}{61.3} & \intrv{139.6}{2255.1}{127.6} & \intrv{74.3}{8387.6}{66.6} & \intrv{284.0}{7544.7}{255.3} & \intrv{45.3}{4726.3}{40.1} & \intrv{261.7}{6542.9}{249.2} & \intrv{72.8}{2764.6}{65.1} & \intrv{64.7}{3834.0}{57.8} & \intrv{117.5}{5827.2}{107.2} & \intrv{49.0}{7140.6}{44.1} \\


==> 4_det_subnet.tex <==
& HIKL & HIKV & HILV & HKLV & IKLV \\
\hline
BNS uniform & \intrv{37.7}{107.6}{32.0} & \intrv{20.9}{95.7}{17.8} & \intrv{30.2}{103.7}{25.7} & \intrv{41.3}{525.3}{36.6} & \intrv{21.5}{70.1}{18.2} \\
BNS normal & \intrv{35.7}{94.0}{29.8} & \intrv{20.2}{90.2}{17.1} & \intrv{28.3}{114.1}{24.4} & \intrv{34.1}{435.2}{29.8} & \intrv{18.7}{77.9}{15.8} \\
NSBH uniform & \intrv{94.2}{13416.6}{83.1} & \intrv{55.1}{19966.7}{48.5} & \intrv{90.6}{20429.2}{79.1} & \intrv{139.7}{26320.0}{130.5} & \intrv{58.2}{23497.0}{51.1} \\
NSBH astro & \intrv{52.3}{685.6}{45.3} & \intrv{31.2}{1344.0}{26.4} & \intrv{43.1}{1443.8}{36.4} & \intrv{66.0}{2207.9}{60.2} & \intrv{33.4}{684.1}{29.0} \\


==> 5_det_subnet.tex <==
& HIKLV \\
\hline
BNS uniform & \intrv{18.3}{50.9}{14.8} \\
BNS normal & \intrv{17.3}{51.6}{14.2} \\
NSBH uniform & \intrv{53.3}{16374.3}{46.4} \\
NSBH astro & \intrv{26.4}{234.2}{22.4} \\


==> 5_inst_above.tex <==
\begin{tabular}{c|cccc|ccc}
\hline
\hline
 & \multicolumn{4}{c|}{\makecell{Network (second generation, \\ two instr. above threshold) \\ $\Omega_{\textrm{90}\%}$ (sq. deg.)}} & \multicolumn{3}{c}{duty cycle} \\
\input{2g_ndet_loc.tex}
\hline
%\end{tabular}

%\begin{tabular}{c|cccc|ccc}
\hline
\hline
 & \multicolumn{4}{c|}{\makecell{Network (second generation, \\ all instr. above threshold) \\ $\Omega_{\textrm{90}\%}$ (sq. deg.)}} & \multicolumn{3}{c}{duty cycle} \\
\input{2g_loc.tex}
\hline

\end{tabular}

\caption{\label{tbl:skyloc_summ}Sky localization result summarized by the median and the symmetric $90\%$ containment values (in sq.\ deg.) of the $90\%$ credible regions. Each network configuration (labeled by $N$) and population (left column) is presented. The columns listed with duty cycles are computed from a set of $N$-fold distributions, weighted by the appropriate factors from the assumed duty cycle, see Equation \eqref{eqn:dcweight}.}
\end{table*}

Table \ref{tbl:skyloc_summ} present differing detected event distributions. The top table requires only that the number of instruments above threshold of 5.5 is two or greater. The bottom one requires that all $N$ instruments are above threshold. The criteria presented here is a reasonable proxy for prompting \emph{examination} of an event. In contrast, the $N$ instrument above threshold criteria allows for a more idealized case, isolating the performance of all instruments when the SNR is high. In what follows, unless explicitly stated, figures display the two instrument thresholding results, so as to best capture what potential event distributions may look like.

There is two orders of magnitude when considering the $5$-fold network ($k=5$) versus $2$-instrument configurations when enforcing that all instruments are above threshold. This gain is reduced to only an order of magnitude for the two-above-threshold strategy. 

The major difference comparing across the table is the role of events which are below threshold in one or more instruments. In this regard, the 2-fold network distributions in either table are identical (differing only statistically). However, the difference as the number of instruments participating increases is dramatic. $k=5$ exhibits a ten-fold shift in the region distribution when going from two or more instruments above threshold to five. The $3$- and $4$-fold network combinations are not as severe, likely because there are fewer ways to obtain events with the same number of instruments below threshold (e.g.. for the $3$-fold network, at most only one instrument can be below threshold). A more complete breakdown of the sub-network performance is in Section \ref{sec:subnets}.

% From conclusions
Attaching the additional condition of have $\rho_{\textrm{net}} > 12$ to the two-above-threshold set reduces medians by a factor of about $2$--$3$ for all network configurations tested, independently of source category or duty cycle. 
For the 2-fold configurations, the other two sets are degenerate, and so this is an overall decrease. As expected, the $5$-fold network median decrease is less pronounced for two-above to the network SNR cut, a little smaller than a factor of two. This should be contrasted with the factor of five obtained for the SNR cut versus the all-above-threshold result. This places the network SNR cut as a middle point between the more inclusive and more optimistic results, when excluding $k=2$. Consequently, the $80\%$ duty cycle result is also about half in the median of the two-above threshold set, but overall three times larger than the all-above threshold set.

